A Renaissance study of Am stars. I. The mass ratio distribution

Triggered by the study of Carquillat & Prieur (2007, MNRAS, 380, 1064) of Am binaries, I reanalyse their sample of 60 orbits to derive the mass ratio distribution (MRD), assuming as they did a priori functional forms, i.e. a power law or a Gaussian. The sample is then extended using orbits published by several groups and a full analysis of the MRD is made, without any assumption on the functional form. I derive the MRD using a Richardson-Lucy inversion method, assuming a fixed mass of the Am primary and randomly distributed orbital inclinations. Using the large sub-sample of double-lined spectroscopic binaries, I show that this methodology is indeed perfectly adequate. Using the inversion method, applied to my extended sample of 162 systems, I find that the final MRD can be approximated by a uniform distribution.

==> graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle
% Slight changes made by Richard Koch

\newif\ifpdf
\ifx\pdfoutput\undefined
\pdffalse % we are not running PDFLaTeX
\else
\pdfoutput=1 % we are running PDFLaTeX
\pdftrue
\fi


\input miniltx

\def\paperheight{11in}
\def\paperwidth{8.5in}
\def\AtEndOfPackage{}
\def\@ifpackageloaded#1{}

\ifpdf
\def\Gin@driver{pdftex.def}
\else
\def\Gin@driver{dvips.def}
\fi

\input graphicx.sty


\resetatcatcode



